SMEFT deviations

This work is based on a bottom{-}up approach to the standard{-}model effective field theory (SMEFT), resulting in an equiprobable space of Wilson coefficients. The randomly generated Wilson coefficients of the SMEFT (in the Warsaw basis) are treated as pseudo-data and, for each observable, the corresponding probability density function is computed. The goal has been to understand how large are the deviations from the SM once the SMEFT scale and the range of the Wilson coefficients are selected. Correlations between different observables are also discussed.

==> SMEFTdev_aux.tex <==
\usepackage[dvipsnames]{xcolor}
%---
\usepackage{graphicx}
\usepackage{amssymb}
\RequirePackage{mathptmx}
\RequirePackage[T1]{fontenc}
%---
\usepackage{heppennames2}
\usepackage{lhchiggs}
\usepackage{cernunits}
%---
\usepackage{pifont}
\usepackage{ctable}
%\usepackage{fancybox}
\usepackage[center,small,bf]{caption}
\usepackage{parskip}
\usepackage{enumerate}
\usepackage{url}
\usepackage[utf8]{inputenc}
%\usepackage{unicode}
%---
% http://en.wikibooks.org/wiki/LaTeX/Hyperlinks
\usepackage[unicode,pagebackref=true]{hyperref}
\hypersetup{ bookmarks=true, % show bookmarks bar? unicode=false, % non-Latin characters in Acrobat?s bookmarks pdftoolbar=true, % show Acrobat?s toolbar? pdfmenubar=true, % show Acrobat?s menu? pdffitwindow=false, % window fit to page when opened pdfstartview={FitH}, % fits the width of the page to the window pdftitle={My title}, % title pdfauthor={Author}, % author pdfsubject={Subject}, % subject of the document pdfcreator={Creator}, % creator of the document pdfproducer={Producer}, % producer of the document pdfkeywords={keyword1} {key2} {key3}, % list of keywords pdfnewwindow=true, % links in new PDF window colorlinks=false, % false: boxed links; true: colored links linkcolor=red, % color of internal links (change box color with linkbordercolor) citecolor=green, % color of links to bibliography filecolor=magenta, % color of file links urlcolor=cyan % color of external links }
%
%\hypersetup{
%    bookmarks=true,         % show bookmarks bar?
%    unicode=true,           % non-Latin characters in Acrobat’s bookmarks
%    pdftoolbar=true,        % show Acrobat’s toolbar?
%    pdfmenubar=true,        % show Acrobat’s menu?
%    pdffitwindow=false,     % window fit to page when opened
%    pdfstartview={FitH},    % fits the width of the page to the window
%    pdftitle={My title},    % title
%    pdfauthor={Author},     % author
%    pdfsubject={Subject},   % subject of the document
%    pdfcreator={Creator},   % creator of the document
%    pdfproducer={Producer}, % producer of the document
%    pdfkeywords={keyword1} {key2} {key3}, % list of keywords
%    pdfnewwindow=true,      % links in new PDF window
%    colorlinks=true,        % false: boxed links; true: colored links
%    linkcolor=blue,         % color of internal links (change box color with linkbordercolor)
%%    citecolor=magenta,       % color of links to bibliography
%    citecolor=OliveGreen,   % color of links to bibliography
%%    filecolor=magenta,     % color of file links
%    filecolor=Mahogany,     % color of file links
%    urlcolor=RoyalBlue      % color of external links
%%    urlcolor=cyan           % color of external links
}
\renewcommand*\backref[1]{\ifx#1\relax \else (#1) \fi}
\biboptions{square,numbers,sort&compress}
% \usepackage[square,numbers,sort&compress]{natbib}
 \usepackage{hypernat}
%---
%---
\hyphenation{ma-ni-pu-la-tions}
\allowdisplaybreaks
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% basic data for the eprint:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textwidth=6.5in  \textheight=8.7in
% \leftmargin=-0.8in   \topmargin=-0.20in
% \hoffset=-.85in

%% preprint number data:
%% Change the preprint number below to your institutional preprint number
\newcommand\pubdate{\today}
%% If you will submit to hep-ex, change hep-ph to hep-ex below
%% Do not change yymmnnn; this will be automatically converted
%% to the Los Alamos hep number during the submission process
\newcommand\hepnumber{hep-ph/yymmnnn}

%%  address and funding acknowledgment data:
\def\csumb{Dipartimento di Fisica Teorica, Universit\`a di Torino, Italy\\
           INFN, Sezione di Torino, Italy}
\def\csuma{Albert-Ludwigs-Universit\"at Freiburg, Physikalisches Institut\\
           D-79104, Freiburg, Germany}
\def\csumc{INFN, Sezione di Torino, Italy}
%\def\support{Work supported by MIUR under contract
%    2001023713$\_$006 and by the Research Executive Agency (REA) of the European Union
%under the Grant Agreement PITN-GA-2012-316704 (HiggsTools).}
\def\support{Work supported by the Research Executive Agency (REA) of the European Union
under the Grant Agreement PITN-GA-2012-316704 (HiggsTools).}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   document style macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\Title#1{\begin{center} {\Large\bf #1 } \end{center}}
\newcommand{\Authors}[2]{\begin{center}{ \sc #1 \hspace{0.1cm} {\rm and}
\hspace{0.1cm} #2} \end{center}}
\def\Author#1{\begin{center}{ \sc #1} \end{center}}
\def\Address#1{\begin{center}{ \it #1} \end{center}}
\def\andauth{\begin{center}{and} \end{center}}
\def\submit#1{\begin{center}Submitted to {\sl #1} \end{center}}
\newcommand\pubblock{\rightline{\begin{tabular}{l} \\
         \pubdate\\  \end{tabular}}}
\newenvironment{Abstract}{\begin{quotation}  }{\end{quotation}}
\newenvironment{Presented}{\begin{quotation} \begin{center}
             Presented at the\end{center}
      \begin{center}\begin{large}}{\end{large}\end{center} \end{quotation}}
\def\Acknowledgments{\bigskip  \bigskip \begin{center}
          \large\bf Acknowledgments\end{center}}
%\def\email#1{\footnote{\color{NavyBlue}{#1}}}
%
\def\email#1{\footnote{\href{mailto:#1}{#1}}}
%
\makeatletter
\def\section{\@startsection{section}{0}{\z@}{5.5ex plus .5ex minus
 1.5ex}{2.3ex plus .2ex}{\large\bf}}
\def\subsection{\@startsection{subsection}{1}{\z@}{3.5ex plus .5ex minus
 1.5ex}{1.3ex plus .2ex}{\normalsize\bf}}
\def\subsubsection{\@startsection{subsubsection}{2}{\z@}{-3.5ex plus
-1ex minus  -.2ex}{2.3ex plus .2ex}{\normalsize\sl}}
%\titleformat{\paragraph}[runin]{\normalfont\normalsize\bfseries}{}{0pt}{}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% small size table and figure captions %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\@makecaption}[2]{%
   \vskip 10pt
   \setbox\@tempboxa\hbox{\small #1: #2}
   \ifdim \wd\@tempboxa >\hsize     % IF longer than one line:
       \small #1: #2\par          %   THEN set as ordinary paragraph.
     \else                        %   ELSE  center.
       \hbox to\hsize{\hfil\box\@tempboxa\hfil}
   \fi}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% macros to collapse citation numbers to ranges %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \citenum emits the plain citation number without ornament
% \citea puts it's argument into the ornamentation for citations
% thus \cite{foo} is equivalent to \citea{\citenum{foo}}
 \def\citenum#1{{\def\@cite##1##2{##1}\cite{#1}}}
\def\citea#1{\@cite{#1}{}}
%
% Collapse citation numbers to ranges.  Non-numeric and undefined labels
% are handled.  No sorting is done.  E.g., 1,3,2,3,4,5,foo,1,2,3,,4,5
% gives 1,3,2-5,foo,1-3,,4,5
\newcount\@tempcntc
\def\@citex[#1]#2{\if@filesw\immediate\write\@auxout{\string\citation{#2}}\fi
  \@tempcnta\z@\@tempcntb\m@ne\def\@citea{}\@cite{\@for\@citeb:=#2\do
    {\@ifundefined
       {b@\@citeb}{\@citeo\@tempcntb\m@ne\@citea\def\@citea{,}{\bf }\@warning
       {Citation `\@citeb' on page \thepage \space undefined}}%
    {\setbox\z@\hbox{\global\@tempcntc0\csname b@\@citeb\endcsname\relax}%
     \ifnum\@tempcntc=\z@ \@citeo\@tempcntb\m@ne
       \@citea\def\@citea{,}\hbox{\csname b@\@citeb\endcsname}%
     \else
      \advance\@tempcntb\@ne
      \ifnum\@tempcntb=\@tempcntc
      \else\advance\@tempcntb\m@ne\@citeo
      \@tempcnta\@tempcntc\@tempcntb\@tempcntc\fi\fi}}\@citeo}{#1}}
\def\@citeo{\ifnum\@tempcnta>\@tempcntb\else\@citea\def\@citea{,}%
  \ifnum\@tempcnta=\@tempcntb\the\@tempcnta\else
  {\advance\@tempcnta\@ne\ifnum\@tempcnta=\@tempcntb \else\def\@citea{--}\fi
    \advance\@tempcnta\m@ne\the\@tempcnta\@citea\the\@tempcntb}\fi\fi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% corrects bad spacing in LaTeX multiple line equations
% replace eqnarray with Eanarray (or use abbreviations
% in econfmacros2.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newenvironment{Eqnarray}%
%   {\arraycolsep 0.14em\begin{eqnarray}}{\end{eqnarray}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  personal abbreviations and macros
%    the following package contains macros used in this document:
%--
%- Local macros
%--
\DeclareRobustCommand{\PA}{\HepParticle{A}{}{}\Xspace}
\DeclareRobustCommand{\PV}{\HepParticle{V}{}{}\Xspace}
\DeclareRobustCommand{\PX}{\HepParticle{X}{}{}\Xspace}
\DeclareRobustCommand{\PY}{\HepParticle{Y}{}{}\Xspace}
\DeclareRobustCommand{\Pf}{\HepParticle{f}{}{}\Xspace}
\DeclareRobustCommand{\PAf}{\HepAntiParticle{\Pf}{}{}\Xspace}
\DeclareRobustCommand{\PF}{\HepParticle{F}{}{}\Xspace}
\DeclareRobustCommand{\PI}{\HepParticle{I}{}{}\Xspace}
\DeclareRobustCommand{\PL}{\HepParticle{L}{}{}\Xspace}
\DeclareRobustCommand{\PG}{\HepParticle{G}{}{}\Xspace}
\DeclareRobustCommand{\PS}{\HepParticle{S}{}{}\Xspace}
\DeclareRobustCommand{\PGN}{\HepParticle{N}{}{}\Xspace}
\DeclareRobustCommand{\Phad}{\HepParticle{h}{}{}\Xspace}
\DeclareRobustCommand{\Pho}{\HepParticle{h}{1}{}\Xspace}
\DeclareRobustCommand{\Pht}{\HepParticle{h}{2}{}\Xspace}
\DeclareRobustCommand{\PQQ}{\HepParticle{Q}{}{}\Xspace}
\DeclareRobustCommand{\PQU}{\HepParticle{U}{}{}\Xspace}
\DeclareRobustCommand{\PQD}{\HepParticle{D}{}{}\Xspace}
\DeclareRobustCommand{\PP}{\HepParticle{P}{}{}\Xspace}
%
\newcommand{\PHH}{\PH\PH}
\newcommand{\PAA}{\PA\PA}
\newcommand{\PAZ}{\PA\PZ}
\newcommand{\PZA}{\PZ\PA}
\newcommand{\PZZ}{\PZ\PZ}
\newcommand{\PWW}{\PW\PW}
\newcommand{\PVV}{\PV\PV}
%
\newcommand{\AT}{\mathrm{\scriptscriptstyle{AT}}}
\newcommand{\TG}{\mathrm{\scriptscriptstyle{TG}}}
\newcommand{\LG}{\mathrm{\scriptscriptstyle{LG}}}
\newcommand{\EFT}{\rm{\scriptscriptstyle{EFT}}}
\newcommand{\XEFT}{\rm{\scriptscriptstyle{XEFT}}}
\newcommand{\SMP}{SM${}^{\prime}$}
\newcommand{\SMEFT}{\rm{\scriptscriptstyle{SMEFT}}}
\newcommand{\HEFT}{\rm{\scriptscriptstyle{HEFT}}}
\newcommand{\QEDEFT}{\rm{\scriptscriptstyle{QEDEFT}}}
\newcommand{\THDM}{\rm{\scriptscriptstyle{THDM}}}
\newcommand{\FR}{\rm{\scriptscriptstyle{FR}}}
\newcommand{\myLO}{\mathrm{\scriptscriptstyle{LO}}}
\newcommand{\myNLO}{\mathrm{\scriptscriptstyle{NLO}}}
\newcommand{\myNNLO}{\mathrm{\scriptscriptstyle{NNLO}}}
\newcommand{\myQCD}{\mathrm{\scriptscriptstyle{QCD}}}
\newcommand{\PTG}{\mathrm{\scriptscriptstyle{PTG}}}
\newcommand{\mix}{\mathrm{\scriptscriptstyle{mix}}}
%\newcommand{\LG}{\mathrm{\scriptscriptstyle{LG}}}
\newcommand{\CT}{\mathrm{CT}}
\newcommand{\dZ}{\mathrm{dZ}}
\newcommand{\OS}{\mathrm{OS}}
\newcommand{\myQED}{\mathrm{QED}}
\newcommand{\CPP}{\mathrm{CPP}}
\newcommand{\mUV}{\mathrm{UV}}
\newcommand{\mBW}{\mathrm{BW}}
\newcommand{\OFS}{\mathrm{OFS}}
\newcommand{\intf}{\mathrm{int}}
\newcommand{\mySM}{\rm{\scriptscriptstyle{SM}}}
\newcommand{\sUV}{\rm{\scriptscriptstyle{UV}}}
\newcommand{\sIR}{\rm{\scriptscriptstyle{IR}}}
\newcommand{\epIR}{\frac{1}{2}\,\ep_{\sIR}}
\newcommand{\BSM}{\rm{\scriptscriptstyle{BSM}}}
\newcommand{\SESM}{\rm{\scriptscriptstyle{SESM}}}
\newcommand{\myEW}{{\scriptscriptstyle{E}\scriptscriptstyle{W}}}
\newcommand{\ssA}{{\mathrm{A}}}
\newcommand{\ssB}{{\mathrm{B}}}
\newcommand{\ssC}{{\mathrm{C}}}
\newcommand{\ssQ}{{\mathrm{Q}}}
\newcommand{\ssE}{{\mathrm{E}}}
\newcommand{\ssF}{{\mathrm{F}}}
\newcommand{\ssG}{{\mathrm{G}}}
\newcommand{\ssR}{{\mathrm{R}}}
\newcommand{\ssK}{{\mathrm{K}}}
\newcommand{\ssdR}{{\mathrm{dR}}}
\newcommand{\ssdZ}{{\mathrm{dZ}}}
\newcommand{\ssdCZ}{{\mathrm{d}{\mathcal{Z}}}}
\newcommand{\ssD}{{\mathrm{D}}}
\newcommand{\ssI}{{\mathrm{I}}}
\newcommand{\ssU}{{\mathrm{U}}}
\newcommand{\ssL}{{\mathrm{L}}}
\newcommand{\ssP}{{\mathrm{P}}}
\newcommand{\ssPR}{{\mathrm{PR}}}
\newcommand{\ssOS}{{\mathrm{OS}}}
\newcommand{\ssS}{{\mathrm{S}}}
\newcommand{\ssH}{{\mathrm{H}}}
\newcommand{\ssV}{{\mathrm{V}}}
\newcommand{\ssM}{{\mathrm{M}}}
\newcommand{\ssN}{{\mathrm{N}}}
\newcommand{\ssX}{{\mathrm{X}}}
\newcommand{\ssY}{{\mathrm{Y}}}
\newcommand{\sH}{\mathrm{H}}
\newcommand{\HH}{\mathrm{HH}}
\newcommand{\VV}{\mathrm{VV}}
\newcommand{\TR}{\mathrm{TR}}
\newcommand{\ssh}{{\mathrm{h}}}
\newcommand{\mra}{{\mathrm{a}}\,}
\newcommand{\mrb}{{\mathrm{b}}}
\newcommand{\mrc}{{\mathrm{c}}}
\newcommand{\mrd}{{\mathrm{d}}}
\newcommand{\mre}{{\mathrm{e}}}
\newcommand{\mrh}{{\mathrm{h}}}
\newcommand{\mrab}{{\overline{\mathrm{a}}}\,}
\newcommand{\mrat}{{\hat{\mathrm{a}}}\,}
\newcommand{\hH}{{\hat{\mathrm{H}}}}
\newcommand{\hpsi}{{\hat{\uppsi}}}
\newcommand{\hchi}{{\hat{\upchi}}}
\newcommand{\hA}{{\hat{\mathrm{A}}}}
\newcommand{\hM}{{\hat{M}}}
\newcommand{\hg}{{\hat{g}}}
\newcommand{\hats}{{\hat{s}}}
\newcommand{\hatt}{{\hat{t}}}
\newcommand{\hMH}{{\hat{M}_{\mrH}}}
%\newcommand{\mrc}{{\mathrm{c}}}
%\newcommand{\mrd}{{\mathrm{d}}}
\newcommand{\mri}{{\mathrm{i}}}
\newcommand{\mrg}{{\mathrm{g}}}
\newcommand{\mrl}{{\mathrm{l}}}
\newcommand{\mrm}{{\mathrm{m}}}
\newcommand{\mrn}{{\mathrm{n}}}
\newcommand{\mrs}{{\mathrm{s}}}
\newcommand{\mrv}{{\mathrm{v}}}
\newcommand{\mru}{{\mathrm{u}}}
\newcommand{\mrr}{{\mathrm{r}}}
\newcommand{\mrx}{{\mathrm{x}}}
\newcommand{\mry}{{\mathrm{y}}}
\newcommand{\mrz}{{\mathrm{z}}}
\newcommand{\mrp}{{\mathrm{p}}}
\newcommand{\mrq}{{\mathrm{q}}}
\newcommand{\mrt}{{\mathrm{t}}}
\newcommand{\mrf}{{\mathrm{f}}}
\newcommand{\ssW}{{\mathrm{W}}}
\newcommand{\ssWF}{{\mathrm{WF}}}
\newcommand{\ssWW}{{\scriptscriptstyle{\PWW}}}
\newcommand{\ssZZ}{{\scriptscriptstyle{\PZZ}}}
\newcommand{\ssT}{{\mathrm{T}}}
\newcommand{\ssZ}{{\mathrm{Z}}}
\newcommand{\bqas}{\begin{eqnarray*}}
\newcommand{\eqas}{\end{eqnarray*}}
\newcommand{\nl}{\nonumber\\}
\newcommand{\nlr}{\right.\nonumber\\}
\newcommand{\cnt}[1]{{}&#1& \left.}
\def\mnew{\mpar{\hfil NEW \hfil}\ignorespaces}
\newcommand{\lpar}{\left(}                            % bracketing
\newcommand{\rpar}{\right)}
\newcommand{\lbra}{\left[\Xspace}
\newcommand{\rbra}{\Xspace\right]}
\newcommand{\lcbr}{\left\{}
\newcommand{\rcbr}{\right\}}
\newcommand{\rbrak}[1]{\lrbr#1\rrbr}
\newcommand{\bq}{\begin{equation}}                    % equationing
\newcommand{\eq}{\end{equation}}
\newcommand{\bqa}{\arraycolsep 0.14em\begin{eqnarray}}
\newcommand{\eqa}{\end{eqnarray}}
\newcommand{\ba}[1]{\begin{array}{#1}}
\newcommand{\ea}{\end{array}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\bei}{\begin{itemize}}
\newcommand{\eei}{\end{itemize}}
\newcommand{\eqn}[1]{Eq.(\ref{#1})}
\newcommand{\eqns}[2]{Eqs.(\ref{#1})--(\ref{#2})}
\newcommand{\eqnss}[1]{Eqs.(\ref{#1})}
\newcommand{\eqnsc}[2]{Eqs.(\ref{#1}) and (\ref{#2})}
\newcommand{\eqnst}[3]{Eqs.(\ref{#1}), (\ref{#2}) and (\ref{#3})}
\newcommand{\eqnsf}[4]{Eqs.(\ref{#1}), (\ref{#2}), (\ref{#3}) and (\ref{#4})}
\newcommand{\eqnsv}[5]{Eqs.(\ref{#1}), (\ref{#2}), (\ref{#3}), (\ref{#4}) and (\ref{#5})}
\newcommand{\tbn}[1]{Tab.~\ref{#1}}
\newcommand{\tabn}[1]{Tab.~\ref{#1}}
\newcommand{\tbns}[2]{Tabs.~\ref{#1}--\ref{#2}}
\newcommand{\tabns}[2]{Tabs.~\ref{#1}--\ref{#2}}
\newcommand{\tabnsc}[2]{Tabs.~\ref{#1} and \ref{#2}}
\newcommand{\fig}[1]{Fig.~\ref{#1}}
\newcommand{\figs}[2]{Figs.~\ref{#1}--\ref{#2}}
\newcommand{\sect}[1]{Section~\ref{#1}}
\newcommand{\sects}[2]{Section~\ref{#1} and \ref{#2}}
\newcommand{\sectm}[2]{Section~\ref{#1} -- \ref{#2}}
\newcommand{\subsect}[1]{Subsection~\ref{#1}}
\newcommand{\subsectm}[2]{Subsection~\ref{#1} -- \ref{#2}}
\newcommand{\appendx}[1]{Appendix~\ref{#1}}
%\newcommand{\hsp}{\hspace{.5mm}}
\def\negs{\hspace{-0.26in}}
\def\negsh{\hspace{-0.13in}}
%--
\newcommand{\hatp}{{\hat p}}
\newcommand{\barphi}{\overline{\upphi}}
\newcommand{\baruppsi}{\overline{\uppsi}}
\newcommand{\oeta}{{\overline{\upeta}}}
\newcommand{\barg}{\overline{g}}
\newcommand{\barm}{\overline{m}}
\newcommand{\barq}{\overline q}
\newcommand{\barb}{\overline b}
\newcommand{\bmid}{\Bigr|}
\newcommand{\intrp}{\int_0^{\infty}}
\newcommand{\intMB}{\int_{-i\,\infty}^{+i\,\infty}}
\newcommand{\ord}[1]{{\cal O}\lpar#1\rpar}
\newcommand{\oD}{{\overline \Delta}}
\newcommand{\hD}{{\hat{\Delta}}}
%--
\newcommand{\Mbp}{\mathswitch {m_{\PQbpr}}}
\newcommand{\Mtp}{\mathswitch {m_{\PQtpr}}}
\newcommand{\Mlp}{\mathswitch {m_{\Pl'}}}
\newcommand{\Mnp}{\mathswitch {m_{\PGnl'}}}
\newcommand{\Bref}[1]{Ref.~\cite{#1}}
\newcommand{\Brefs}[1]{Refs.~\cite{#1}}
%
\newcommand{\Fref}[1]{Fig.~\ref[#1]}
\newcommand{\Tref}[1]{Tab.~\ref[#1]}
%--
\newcommand{\eg}{e.g.\xspace}
\newcommand{\ie}{i.e.\xspace}
\newcommand{\etc}{etc.\@\xspace}
\newcommand{\etcc}{etc,\@\xspace}
\newcommand{\etal}{\emph{et al.}}
%\newcommand{\cf}{\emph{cf.\xspace}}
%\newcommand{\SPp}{~}       %% space before punctuation in math
%--
%\newcommand{\mv}{\mathswitch {M_{\ssV}}}
\newcommand{\mv}{\mathswitch{M_{\PV}}}
\newcommand{\mw}{\mathswitch{M_{\PW}}}
\newcommand{\mbw}{\mathswitch{m_{\PW}}}
\newcommand{\mbws}{\mathswitch{m^2_{\PW}}}
\newcommand{\mz}{\mathswitch{M_{\PZ}}}
\newcommand{\mBh}{\mathswitch{{\overline M}_{\PH}}}
\newcommand{\mBhs}{\mathswitch{{\overline M}^2_{\PH}}}
\newcommand{\mws}{\mathswitch{M^2_{\PW}}}
\newcommand{\mwc}{\mathswitch{M^3_{\PW}}}
\newcommand{\mwsOS}{\mathswitch{M^2_{\PW\,;\,\ssOS}}}
\newcommand{\mwq}{\mathswitch{M^4_{\PW}}}
\newcommand{\mwvi}{\mathswitch{M^6_{\PW}}}
\newcommand{\mzs}{\mathswitch{M^2_{\PZ}}}
\newcommand{\mzc}{\mathswitch{M^3_{\PZ}}}
\newcommand{\mzq}{\mathswitch{M^4_{\PZ}}}
\newcommand{\mzOS}{\mathswitch{M_{\PZ\,;\,\ssOS}}}
\newcommand{\mzsOS}{\mathswitch{M^2_{\PZ\,;\,\ssOS}}}
\newcommand{\mt}{\mathswitch{M_{\PQt}}}
\newcommand{\mb}{\mathswitch{M_{\PQb}}}
\newcommand{\mts}{\mathswitch{M^2_{\PQt}}}
\newcommand{\mbs}{\mathswitch{M^2_{\PQb}}}
\newcommand{\mtq}{\mathswitch{M^4_{\PQt}}}
\newcommand{\mbq}{\mathswitch{M^4_{\PQb}}}
\newcommand{\ml}{\mathswitch{M_{\Pl}}}
\newcommand{\me}{\mathswitch{m_{\Pe}}}
\newcommand{\mes}{\mathswitch{m^2_{\Pe}}}
\newcommand{\meq}{\mathswitch{m^4_{\Pe}}}
%
\newcommand{\mUs}{\mathswitch{M^2_{\PQU}}}
\newcommand{\mDs}{\mathswitch{M^2_{\PQD}}}
%
\newcommand{\smh}{\mathswitch{m_{\PH}}}
\newcommand{\mh}{\mathswitch{M_{\PH}}}
\newcommand{\ma}{\mathswitch{M_{\PA}}}
\newcommand{\mhOS}{\mathswitch{M_{\PH\,;\,\ssOS}}}
\newcommand{\mhc}{\mathswitch{M^2_{\sPH}}}
\newcommand{\mhs}{\mathswitch{M^2_{\sPH}}}
\newcommand{\mhsOS}{\mathswitch{M^2_{\PH\,;\,\ssOS}}}
\newcommand{\mhq}{\mathswitch{M^4_{\PH}}}
\newcommand{\mhvi}{\mathswitch{M^6_{\PH}}}
%
\newcommand{\mhr}{\mathswitch{M_{\PH\,\ren}}}
\newcommand{\mhrs}{\mathswitch{M^2_{\PH\,\ren}}}
%
\newcommand{\mqt}{\mathswitch{M_{\PQt}}}
\newcommand{\mqb}{\mathswitch{M_{\PQb}}}
\newcommand{\mqts}{\mathswitch{M^2_{\PQt}}}
\newcommand{\mqbs}{\mathswitch{M^2_{\PQb}}}
\newcommand{\mqtq}{\mathswitch{M^4_{\PQt}}}
\newcommand{\mqbq}{\mathswitch{M^4_{\PQb}}}
%
\newcommand{\sPg}{{\scriptscriptstyle{\Pg}}}
\newcommand{\sPF}{{\scriptscriptstyle{\PF}}}
\newcommand{\sPQQ}{{\scriptscriptstyle{\PQQ}}}
\newcommand{\sPL}{{\scriptscriptstyle{\PL}}}
\newcommand{\sPQU}{{\scriptscriptstyle{\PQU}}}
\newcommand{\sPQD}{{\scriptscriptstyle{\PQD}}}
\newcommand{\sPH}{{\scriptscriptstyle{\PH}}}
\newcommand{\sPh}{{\scriptscriptstyle{\Ph}}}
\newcommand{\sPHpm}{{\scriptscriptstyle{\PHpm}}}
\newcommand{\sPS}{{\scriptscriptstyle{\PS}}}
\newcommand{\sPO}{{\scriptscriptstyle{\PO}}}
\newcommand{\sPM}{{\scriptscriptstyle{\PM}}}
\newcommand{\sPZ}{{\scriptscriptstyle{\PZ}}}
\newcommand{\sPW}{{\scriptscriptstyle{\PW}}}
\newcommand{\sPA}{{\scriptscriptstyle{\PA}}}
\newcommand{\sPB}{{\scriptscriptstyle{\PB}}}
\newcommand{\sPD}{{\scriptscriptstyle{\PD}}}
\newcommand{\sPP}{{\scriptscriptstyle{\PP}}}
\newcommand{\sPV}{{\scriptscriptstyle{\PV}}}
\newcommand{\sPX}{{\scriptscriptstyle{\PX}}}
\newcommand{\sPVV}{{\scriptscriptstyle{\PV\PV}}}
\newcommand{\sPZZ}{{\scriptscriptstyle{\PZZ}}}
\newcommand{\sPWW}{{\scriptscriptstyle{\PWW}}}
\newcommand{\sPWB}{{\scriptscriptstyle{\PW\PB}}}
\newcommand{\sPHAA}{{\scriptscriptstyle{\PH\PAA}}}
\newcommand{\sPHAZ}{{\scriptscriptstyle{\PH\PA\PZ}}}
\newcommand{\sPHAV}{{\scriptscriptstyle{\PH\PA\PV}}}
\newcommand{\sPHZZ}{{\scriptscriptstyle{\PH\PZ\PZ}}}
\newcommand{\sPHWW}{{\scriptscriptstyle{\PH\PW\PW}}}
\newcommand{\sPHVV}{{\scriptscriptstyle{\PH\PV\PV}}}
%
\newcommand{\smu}{\mathswitch{m_{\PQu}}}
\newcommand{\smU}{\mathswitch{m_{\sPQU}}}
\newcommand{\mqu}{\mathswitch{M_{\PQu}}}
\newcommand{\mqU}{\mathswitch{M_{\sPQU}}}
\newcommand{\mqus}{\mathswitch{M^2_{\PQu}}}
\newcommand{\mquq}{\mathswitch{M^4_{\PQu}}}
\newcommand{\mqd}{\mathswitch{M_{\PQd}}}
\newcommand{\mqD}{\mathswitch{M_{\sPQD}}}
\newcommand{\smd}{\mathswitch{m_{\PQd}}}
\newcommand{\smD}{\mathswitch{m_{\sPQD}}}
\newcommand{\mqds}{\mathswitch{M^2_{\PQd}}}
\newcommand{\mqdq}{\mathswitch{M^4_{\PQd}}}
\newcommand{\smLe}{\mathswitch{m_{\sPL}}}
\newcommand{\smle}{\mathswitch{m_{\Pl}}}
\newcommand{\mle}{\mathswitch{M_{\Pl}}}
\newcommand{\mLe}{\mathswitch{M_{\sPL}}}
\newcommand{\mLes}{\mathswitch{M^2_{\sPL}}}
\newcommand{\mles}{\mathswitch{M^2_{\Pl}}}
\newcommand{\mleq}{\mathswitch{M^4_{\Pl}}}
%
\newcommand{\cph}{\mathswitch{s_{\sPH}}}
\newcommand{\cpw}{\mathswitch{s_{\sPW}}}
\newcommand{\cpwz}{\mathswitch{s_{\PW}, s_{\PZ}}}
\newcommand{\cpz}{\mathswitch{s_{\sPZ}}}
\newcommand{\cpt}{\mathswitch{s_{\PQt}}}
\newcommand{\muh}{\mathswitch{\mu_{\PH}}}
\newcommand{\muph}{\mathswitch{\mu'_{\PH}}}
\newcommand{\muhs}{\mathswitch{\mu^2_{\PH}}}
\newcommand{\omuhs}{\mathswitch{{\hat\mu}^2_{\PH}}}
\newcommand{\gh}{\mathswitch{\gamma_{\PH}}}
\newcommand{\emc}{\mathswitch{\gamma}}
\newcommand{\emcb}{\mathswitch{{\overline{\gamma}}}}
\newcommand{\GOS}{\mathswitch{\Gamma_{\OS}}}
\newcommand{\GOL}{\mathswitch{\overline\Gamma}}
\newcommand{\muol}{\mathswitch{\overline\mu}}
\newcommand{\GOSu}{\mathswitch{\Gamma^{\OS}}}
\newcommand{\shat}{\mathswitch{\hat s}}
\newcommand{\muR}{\mathswitch{\mu_{\ssR}}}
\newcommand{\muF}{\mathswitch{\mu_{\ssF}}}
\newcommand{\muRs}{\mathswitch{\mu^2_{\ssR}}}
\newcommand{\muFs}{\mathswitch{\mu^2_{\ssF}}}
\newcommand{\tot}{{\mbox{\scriptsize tot}}}
\newcommand{\myprod}{{\mbox{\scriptsize prod}}}
%%%%\newcommand{\prop}{{\mbox{\scriptsize prop}}}
\newcommand{\proc}{{\mbox{\scriptsize proc}}}
\newcommand{\dec}{{\mbox{\scriptsize dec}}}
\newcommand{\off}{{\mbox{\scriptsize off}}}
\newcommand{\obs}{{\mbox{\scriptsize obs}}}
\newcommand{\kcut}{{\mbox{\scriptsize cut}}}
\newcommand{\bck}{{\mbox{\scriptsize NR}}}
\newcommand{\res}{{\mbox{\scriptsize R}}}
\newcommand{\mysoft}{{\mbox{\scriptsize soft}}}
\newcommand{\ch}{{\mbox{\scriptsize ch}}}
\newcommand{\inv}{{\mbox{\scriptsize inv}}}
\newcommand{\bos}{{\mbox{\scriptsize bos}}}
\newcommand{\peak}{{\mbox{\scriptsize peak}}}
\newcommand{\heavy}{{\mbox{\scriptsize{heavy}}}}
\newcommand{\add}{{\mbox{\scriptsize add}}}
\newcommand{\eff}{{\mbox{\scriptsize eff}}}
\newcommand{\red}{{\mbox{\scriptsize red}}}
\newcommand{\bfm}{{\mbox{\scriptsize bfm}}}
\newcommand{\rest}{{\mbox{\scriptsize rest}}}
\newcommand{\bare}{{\mbox{\scriptsize bare}}}
\newcommand{\tree}{{\mbox{\scriptsize tree}}}
\newcommand{\icdiv}{{\mbox{\scriptsize div}}}
\newcommand{\ppart}{{\mbox{\scriptsize pole}}}
\newcommand{\oL}{{\mbox{\scriptsize 1L}}}
\newcommand{\real}{{\mbox{\scriptsize real}}}
\newcommand{\myvirt}{{\mbox{\scriptsize virt}}}
\newcommand{\loc}{{\mbox{\scriptsize{loc}}}}
\newcommand{\nloc}{{\mbox{\scriptsize{nloc}}}}
%\newcommand{\fin}{{\mbox{\scriptsize fin}}}
\newcommand{\inte}{{\mbox{\scriptsize int}}}
\newcommand{\fin}{{\mbox{\tiny fin}}}
\newcommand{\pole}{{\mbox{\tiny div}}}
\newcommand{\gen}{{\mbox{\scriptsize gen}}}
\newcommand{\ggen}{{\mbox{\tiny gen}}}
\newcommand{\ren}{{\mbox{\scriptsize ren}}}
\newcommand{\ct}{{\mbox{\scriptsize ct}}}
\newcommand{\mdiv}{{\mbox{\scriptsize div}}}
\newcommand{\bin}{{\mbox{\scriptsize in}}}
\newcommand{\bout}{{\mbox{\scriptsize out}}}
\newcommand{\ac}{{\mbox{\scriptsize all}}}
\newcommand{\HO}{{\mathrm{HO}}}
\newcommand{\intfxy}[2]{\int_{\scriptstyle 0}^{\scriptstyle 1}\,d#1\,
                        \int_{\scriptstyle 0}^{\scriptstyle #1}\,d#2}
\newcommand{\li}[2]{\mathrm{Li}_{#1}\lpar\displaystyle{#2}\rpar} % polylog
%--
\newcommand{\eG}[1]{\mathswitch \Gamma\lpar #1 \rpar}
\newcommand{\eGs}[1]{\mathswitch \Gamma^2\lpar #1 \rpar}
\newcommand{\ep}{\mathswitch \varepsilon}
\newcommand{\epb}{\mathswitch{\overline\varepsilon}}
\newcommand{\epbM}{\mathswitch{\overline\varepsilon}_{\mrM}}
\newcommand{\eph}{\mathswitch{\hat\varepsilon}}
\newcommand{\spro}[2]{{#1}\cdot{#2}}
\providecommand\HTO{{\sc HTO}}
\providecommand\POWHEG{{\sc POWHEG}}
\providecommand\iHixs{{\sc iHixs}}
%--
\newcommand{\Srest}[2]{\sigma_{#1}\lpar{#2}\rpar}
\newcommand{\Gdist}[1]{{\mathcal{G}}\lpar{#1}\rpar}
\newcommand{\resolw}{\sigma_{\ssE}}
\newcommand{\resolws}{\sigma^2_{\ssE}}
\newcommand{\ddel}[1]{\delta\lpar#1\rpar}
\newcommand{\Gloni}[1]{\Gamma_{#1}}
\newcommand{\Aareai}[1]{{\mathcal{A}}\lpar{#1}\rpar}
\newcommand{\lrbr}{\left[}
\newcommand{\rrbr}{\right]}
%\newcommand{\lcbr}{\left\{}
%\newcommand{\rcbr}{\right\}}
\newcommand{\sGdist}{{\mathcal{G}}}
\newcommand{\sAarea}{{\mathcal{A}}}
%--
\newcommand{\Ds}{{\mathrm{D}}}
\newcommand{\mrS}{{\mathrm{S}}}
\newcommand{\mrA}{{\mathrm{A}}}
%\newcommand{\mrA}{{{\overline{\mathrm{A}}}}}
\newcommand{\mrB}{{\mathrm{B}}}
\newcommand{\mrC}{{\mathrm{C}}}
\newcommand{\mrD}{{\mathrm{D}}}
\newcommand{\mrE}{{\mathrm{E}}}
\newcommand{\mrF}{{\mathrm{F}}}
\newcommand{\mrG}{{\mathrm{G}}}
\newcommand{\mrH}{{\mathrm{H}}}
\newcommand{\mrI}{{\mathrm{I}}}
\newcommand{\mrJ}{{\mathrm{J}}}
\newcommand{\mrK}{{\mathrm{K}}}
\newcommand{\mrL}{{\mathrm{L}}}
\newcommand{\mrM}{{\mathrm{M}}}
\newcommand{\mrN}{{\mathrm{N}}}
\newcommand{\mrO}{{\mathrm{O}}}
\newcommand{\mrP}{{\mathrm{P}}}
\newcommand{\mrQ}{{\mathrm{Q}}}
\newcommand{\mrR}{{\mathrm{R}}}
%\newcommand{\mrS}{{\mathrm{S}}}
\newcommand{\mrT}{{\mathrm{T}}}
\newcommand{\mrU}{{\mathrm{U}}}
\newcommand{\mrV}{{\mathrm{V}}}
\newcommand{\mrW}{{\mathrm{W}}}
\newcommand{\mrw}{{\mathrm{w}}}
\newcommand{\mrX}{{\mathrm{X}}}
\newcommand{\mrLEX}{{\mathrm{LEX}}}
\newcommand{\mrY}{{\mathrm{Y}}}
\newcommand{\mrZ}{{\mathrm{Z}}}
%\newcommand{\mrW}{{\mathrm{W}}}
%--
\newcommand{\Lcol}{{\mrL_c}}
\newcommand{\LM}{{\mrL}}
%
\newcommand{\Kfac}[2]{\mathrm{K}^{#1}_{#2}}
\newcommand{\Kf}{\mathrm{K}}
\newcommand{\SpI}{\mathrm{S} + \mathrm{I}}
\newcommand{\mfs}{\mathswitch{M_{\Pf}}}
%--
\newcommand{\snitem}{{\tiny{\ding{109}}}\Xspace}
\newcommand{\cmark}{\ding{51}\Xspace}
\newcommand{\ccmark}{\ding{55}\Xspace}
\newcommand{\quo}{\ding{125}\Xspace}
\newcommand{\uquo}{\ding{126}\Xspace}
\newcommand{\bhand}{{\Large{\ding{42}}}\Xspace}
\newcommand{\whand}{{\Large{\ding{43}}}\Xspace}
\newcommand{\vict}{{\Large{\ding{44}}}\Xspace}
\newcommand{\far}{{\Large{\ding{243}}}\Xspace}
\newcommand{\dstar}{{\Large{\ding{85}}}\Xspace}
\newcommand{\apdown}{{\Large{\ding{244}}}\Xspace}
\newcommand{\sciss}{{\Large{\ding{34}}}\Xspace}
\newcommand{\dcross}{{\Huge{\ding{54}}}\Xspace}
\newcommand{\pwrite}{{\Huge{\ding{46}}}\Xspace}
%
\providecommand{\dnuma}{{\Large{\ding{172}}}\Xspace}
\providecommand{\dnumb}{{\Large{\ding{173}}}\Xspace}
\providecommand{\dnumc}{{\Large{\ding{174}}}\Xspace}
\providecommand{\dnumd}{{\Large{\ding{175}}}\Xspace}
\providecommand{\dnume}{{\Large{\ding{176}}}\Xspace}
%--
\providecommand{\dnumA}{{\Large{\ding{182}}}\Xspace\Xspace}
\providecommand{\dnumB}{{\Large{\ding{183}}}\Xspace\Xspace}
%--
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
%
\newenvironment{proof}[1][Proof]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{definition}[1][Definition]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{example}[1][Example]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{remark}[1][Remark]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollary}
%
%\newenvironment{proof}[1][Proof]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{definition}[1][Definition]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{example}[1][Example]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{remark}[1][Remark]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{claim}[1][Claim]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%
\newcommand{\Lag}{{\mathcal{L}}}
\newcommand{\Ope}{{\mathcal{O}}}
\newcommand{\Amp}{{\cal M}}
\newcommand{\srt}{\sqrt{2}}
%
\newcommand{\OpWs}{\Ope^{(6)}_{\upphi\,\scriptscriptstyle{\PW}}}
\newcommand{\OpWe}{\Ope^{(8)}_{\upphi\,\scriptscriptstyle{\PW}}}
%
\DeclareRobustCommand{\POppm}{\HepAntiParticle{\upphi}{}{\,\pm}\Xspace}
\DeclareRobustCommand{\POpp}{\HepAntiParticle{\upphi}{}{\,+}\Xspace}
\DeclareRobustCommand{\POpm}{\HepAntiParticle{\upphi}{}{\,-}\Xspace}
\DeclareRobustCommand{\POpz}{\HepAntiParticle{\upphi}{}{\,0}\Xspace}
%--
\DeclareRobustCommand{\Ppp}{\HepParticle{\upphi}{}{+}\Xspace}
\DeclareRobustCommand{\Ppm}{\HepParticle{\upphi}{}{-}\Xspace}
\DeclareRobustCommand{\Pppm}{\HepParticle{\upphi}{}{\pm}\Xspace}
\DeclareRobustCommand{\Ppz}{\HepParticle{\upphi}{}{0}\Xspace}
%
\DeclareRobustCommand{\PAL}{\HepParticle{\mybar{\PL}}{}{}\Xspace}
\DeclareRobustCommand{\PpsiL}{\HepParticle{\uppsi}{L}{}\Xspace}
\DeclareRobustCommand{\PpsiR}{\HepParticle{\uppsi}{R}{}\Xspace}
\DeclareRobustCommand{\POpsiL}{\HepParticle{\mybar{\uppsi}}{L}{}\Xspace}
\DeclareRobustCommand{\POpsiR}{\HepParticle{\mybar{\uppsi}}{R}{}\Xspace}
\DeclareRobustCommand{\PQtR}{\HepParticle{\PQt}{R}{}\Xspace}
\DeclareRobustCommand{\PQbR}{\HepParticle{\PQb}{R}{}\Xspace}
\DeclareRobustCommand{\PQuR}{\HepParticle{\PQu}{R}{}\Xspace}
\DeclareRobustCommand{\PQdR}{\HepParticle{\PQd}{R}{}\Xspace}
\DeclareRobustCommand{\PQqL}{\HepParticle{\PQq}{L}{}\Xspace}
\DeclareRobustCommand{\PlL}{\HepParticle{\Pl}{L}{}\Xspace}
\DeclareRobustCommand{\PlR}{\HepParticle{\Pl}{R}{}\Xspace}
\DeclareRobustCommand{\PLL}{\HepParticle{\PL}{L}{}\Xspace}
\DeclareRobustCommand{\PLR}{\HepParticle{\PL}{R}{}\Xspace}
\DeclareRobustCommand{\PAQqL}{\HepParticle{\PAQq}{L}{}\Xspace}
\DeclareRobustCommand{\PAlL}{\HepParticle{\PAl}{L}{}\Xspace}
\DeclareRobustCommand{\PAlR}{\HepParticle{\PAl}{R}{}\Xspace}
\DeclareRobustCommand{\PALL}{\HepParticle{\PAL}{L}{}\Xspace}
\DeclareRobustCommand{\PAQuR}{\HepParticle{\PAQu}{R}{}\Xspace}
\DeclareRobustCommand{\PAQdR}{\HepParticle{\PAQd}{R}{}\Xspace}
%-
\newcommand{\pumu}{{\partial^{\mu}}}
%\newcommand{\pdmu}{{\partial_{\mu}}}
%\newcommand{\punu}{{\partial^{\nu}}}
\newcommand{\pdnu}{{\partial_{\nu}}}
%
\newcommand{\myGF}{G_{\mrF}}
%
%\DeclareRobustCommand{\PK}{\HepParticle{K}{}{}\Xspace}
%\DeclareRobustCommand{\Pphi}{\HepParticle{\upphi}{}{}\Xspace}
%\DeclareRobustCommand{\PKdag}{\HepParticle{\PK}{}{\dagger}\Xspace}
%\newcommand{\KdK}{\lpar \PKdag\,\PK\rpar }
%
%\DeclareRobustCommand{\PK}{\HepParticle{\upPhi}{}{}\Xspace}
\DeclareRobustCommand{\Pphi}{\HepParticle{\upphi}{}{}\Xspace}
\DeclareRobustCommand{\PKdag}{\HepParticle{\PK}{}{\dagger}\Xspace}
\newcommand{\KdK}{\lpar \PKdag\,\PK\rpar }
%
\DeclareRobustCommand{\Pxi}{\HepParticle{\upxi}{}{}\Xspace}
\DeclareRobustCommand{\Pxip}{\HepParticle{\upxi}{}{+}\Xspace}
\DeclareRobustCommand{\Pxim}{\HepParticle{\upxi}{}{-}\Xspace}
\DeclareRobustCommand{\Pxiz}{\HepParticle{\upxi}{}{0}\Xspace}
\DeclareRobustCommand{\Pxid}{\HepParticle{\upxi}{}{\dagger}\Xspace}
%
\newcommand{\dPK}{{\partial\PK}}
\newcommand{\essV}{{\mathrm{e}\PV}}
\DeclareRobustCommand{\PAf}{\HepAntiParticle{\Pf}{}{}\Xspace}
%
%\newcommand{\mrc}{\mathrm{c}}
%\newcommand{\mrs}{\mathrm{s}}
%
\newcommand{\stse}{\sin\theta^{\Pf}_{\eff}}
%
\newcommand{\sa}{\mrs_{_{\alpha}}}
\newcommand{\ca}{\mrc_{_{\alpha}}}
%
\newcommand{\stw}{\mrs_{_{\theta}}}             % bare, Lagrangian parameters
\newcommand{\ctw}{\mrc_{_{\theta}}}
\newcommand{\stws}{\mrs_{_{\theta}}^2}
\newcommand{\stwc}{\mrs_{_{\theta}}^3}
\newcommand{\ctws}{\mrc_{_{\theta}}^2}
\newcommand{\ctwc}{\mrc_{_{\theta}}^3}
\newcommand{\stwq}{\mrs_{_{\theta}}^4}
\newcommand{\ctwq}{\mrc_{_{\theta}}^4}
\newcommand{\stwvi}{\mrs_{_{\theta}}^6}
\newcommand{\ctwvi}{\mrc_{_{\theta}}^6}
%
\newcommand{\ctwr}{\mrc^{\ren}_{_{\theta}}}
\newcommand{\stwr}{s^{\ren}_{_{\theta}}}
%
\newcommand{\stW}{\mrs_{_{\PW}}}             % bare, Lagrangian parameters
\newcommand{\ctW}{\mrc_{_{\PW}}}
\newcommand{\stWc}{\mrs_{_{\PW}}^3}
\newcommand{\stWs}{\mrs_{_{\PW}}^2}
\newcommand{\ctWs}{\mrc_{_{\PW}}^2}
\newcommand{\ctWc}{\mrc_{_{\PW}}^3}
\newcommand{\stWq}{\mrs_{_{\PW}}^4}
\newcommand{\ctWq}{\mrc_{_{\PW}}^4}
\newcommand{\stWvi}{\mrs_{_{\PW}}^6}
\newcommand{\ctWvi}{\mrc_{_{\PW}}^6}
%--
\newcommand{\ctb}{\overline{\mrc}_{_{\theta}}}
\newcommand{\stb}{\overline{\mrs}_{_{\theta}}}
\newcommand{\ctbs}{\overline{\mrc}^2_{_{\theta}}}
\newcommand{\stbs}{\overline{\mrs}^2_{_{\theta}}}
%
\newcommand\mybar[1]{\ensuremath{\bar{#1}}}
\newcommand\mytil[1]{\ensuremath{\tilde{#1}}}
%
\newcommand{\cth}{{\hat \mrc}_{_{\theta}}}
\newcommand{\sth}{{\hat \mrs}_{_{\theta}}}
\newcommand{\cths}{{\hat \mrc}^2_{_{\theta}}}
\newcommand{\cthc}{{\hat \mrc}^3_{_{\theta}}}
\newcommand{\sths}{{\hat \mrs}^2_{_{\theta}}}
\newcommand{\sthq}{{\hat \mrs}^4_{_{\theta}}}
%
\newcommand{\HSs}{{\Lambda^2}}
%
\DeclareRobustCommand{\PWs}{\HepParticle{\PW}{}{*}\Xspace}
%
\DeclareRobustCommand{\PWp}{\HepParticle{\PW}{}{+}\Xspace}
\DeclareRobustCommand{\PWm}{\HepParticle{\PW}{}{-}\Xspace}
\DeclareRobustCommand{\PWpmmu}{\HepParticle{\PW}{\mu}{\pm}\Xspace}
\DeclareRobustCommand{\PWpmu}{\HepParticle{\PW}{\mu}{+}\Xspace}
\DeclareRobustCommand{\PWmmu}{\HepParticle{\PW}{\mu}{-}\Xspace}
\DeclareRobustCommand{\PWmnu}{\HepParticle{\PW}{\nu}{-}\Xspace}
\DeclareRobustCommand{\PWpnu}{\HepParticle{\PW}{\nu}{+}\Xspace}
\DeclareRobustCommand{\PWmnu}{\HepParticle{\PW}{\nu}{-}\Xspace}
\DeclareRobustCommand{\PZmu}{\HepParticle{\PZ}{\mu}{}\Xspace}
\DeclareRobustCommand{\PAmu}{\HepParticle{\PA}{\mu}{}\Xspace}
\DeclareRobustCommand{\PZnu}{\HepParticle{\PZ}{\nu}{}\Xspace}
\DeclareRobustCommand{\PAnu}{\HepParticle{\PA}{\nu}{}\Xspace}
%
\DeclareRobustCommand{\PAumu}{\HepParticle{\PA}{}{\mu}\Xspace}
\DeclareRobustCommand{\PAdmu}{\HepParticle{\PA}{\mu}{}\Xspace}
%
\DeclareRobustCommand{\PZumu}{\HepParticle{\PZ}{}{\mu}\Xspace}
\DeclareRobustCommand{\PZdmu}{\HepParticle{\PZ}{\mu}{}\Xspace}
%\DeclareRobustCommand{\PZdmus}{\HepParticle{\PZ}{\mu}{}\Xspace}
\DeclareRobustCommand{\PZunu}{\HepParticle{\PZ}{}{\nu}\Xspace}
\DeclareRobustCommand{\PZdnu}{\HepParticle{\PZ}{\nu}{}\Xspace}
%
\DeclareRobustCommand{\PAumu}{\HepParticle{\PA}{}{\mu}\Xspace}
\DeclareRobustCommand{\PAdmu}{\HepParticle{\PA}{\mu}{}\Xspace}
\DeclareRobustCommand{\PAunu}{\HepParticle{\PA}{}{\nu}\Xspace}
\DeclareRobustCommand{\PAdnu}{\HepParticle{\PA}{\nu}{}\Xspace}
%
\DeclareRobustCommand{\PWpumu}{\HepParticle{\PW}{}{+\,\mu}\Xspace}
\DeclareRobustCommand{\PWmdmu}{\HepParticle{\PW}{\mu}{-}\Xspace}
\DeclareRobustCommand{\PWpunu}{\HepParticle{\PW}{}{+\,\nu}\Xspace}
\DeclareRobustCommand{\PWmdnu}{\HepParticle{\PW}{\nu}{-}\Xspace}
%
\DeclareRobustCommand{\PWmumu}{\HepParticle{\PW}{}{-\,\mu}\Xspace}
\DeclareRobustCommand{\PWpdmu}{\HepParticle{\PW}{\mu}{+}\Xspace}
\DeclareRobustCommand{\PWmunu}{\HepParticle{\PW}{}{-\,\nu}\Xspace}
\DeclareRobustCommand{\PWpdnu}{\HepParticle{\PW}{\nu}{+}\Xspace}
%--
\DeclareRobustCommand{\PXpm}{\HepParticle{\PX}{}{\pm}\Xspace}
\DeclareRobustCommand{\PXp}{\HepParticle{\PX}{}{+}\Xspace}
\DeclareRobustCommand{\PXm}{\HepParticle{\PX}{}{-}\Xspace}
\DeclareRobustCommand{\PYz}{\HepParticle{\PY}{\PZ}{}\Xspace}
\DeclareRobustCommand{\PYa}{\HepParticle{\PY}{\PA}{}\Xspace}
%
\DeclareRobustCommand{\PHb}{\HepAntiParticle{\PH}{}{}\Xspace}
\DeclareRobustCommand{\Ppzb}{\HepAntiParticle{\upphi}{}{\,0}\Xspace}
\DeclareRobustCommand{\Pppmb}{\HepAntiParticle{\upphi}{}{\pm}\Xspace}
\DeclareRobustCommand{\PAb}{\HepAntiParticle{\PA}{}{}\Xspace}
\DeclareRobustCommand{\PAbmu}{\HepAntiParticle{\PA}{}{\mu}\Xspace}
\DeclareRobustCommand{\PAbmud}{\HepAntiParticle{\PA}{\mu}{}\Xspace}
\DeclareRobustCommand{\PZb}{\HepAntiParticle{\PZ}{}{}\Xspace}
\DeclareRobustCommand{\PZbmu}{\HepAntiParticle{\PZ}{}{\mu}\Xspace}
\DeclareRobustCommand{\PZbmud}{\HepAntiParticle{\PZ}{\mu}{}\Xspace}
%
\DeclareRobustCommand{\PWpmbmu}{\HepAntiParticle{\PW}{}{\pm\,\mu}\Xspace}
\DeclareRobustCommand{\PWpmbmud}{\HepAntiParticle{\PW}{\mu}{\pm}\Xspace}
\DeclareRobustCommand{\PWb}{\HepAntiParticle{\PW}{}{}\Xspace}
\DeclareRobustCommand{\PWpb}{\HepAntiParticle{\PW}{}{+}\Xspace}
\DeclareRobustCommand{\PWmb}{\HepAntiParticle{\PW}{}{-}\Xspace}
\DeclareRobustCommand{\Pgb}{\HepAntiParticle{\Pg}{}{}\Xspace}
\DeclareRobustCommand{\PQtb}{\HepAntiParticle{\PQt}{}{}\Xspace}
\DeclareRobustCommand{\PQbb}{\HepAntiParticle{\PQb}{}{}\Xspace}
\DeclareRobustCommand{\PXpmb}{\HepAntiParticle{\PX}{}{\pm}\Xspace}
\DeclareRobustCommand{\PYzb}{\HepAntiParticle{\PY}{\PZ}{}\Xspace}
\DeclareRobustCommand{\PYab}{\HepAntiParticle{\PY}{\PA}{}\Xspace}
%
\DeclareRobustCommand{\PAXpm}{\HepAntiParticle{\PX}{}{\,\pm}\Xspace}
\DeclareRobustCommand{\PAXp}{\HepAntiParticle{\PX}{}{\,+}\Xspace}
\DeclareRobustCommand{\PAXm}{\HepAntiParticle{\PX}{}{\,-}\Xspace}
\DeclareRobustCommand{\PAYz}{\HepAntiParticle{\PY}{\,\PZ}{}\Xspace}
\DeclareRobustCommand{\PAYa}{\HepAntiParticle{\PY}{\,\PA}{}\Xspace}
%
\newcommand{\POZ}{{\overline{\PZ}}}
\newcommand{\POA}{{\overline{\PA}}}
\newcommand{\POH}{{\overline{\PH}}}
\newcommand{\POp}{{\overline{\upphi}}}
%--
\DeclareRobustCommand{\PdT}{\HepParticle{\mytil{\PF}}{\mu\nu}{a}\Xspace}
\DeclareRobustCommand{\HB}{\HepAntiParticle{\PH}{}{}\Xspace}
\DeclareRobustCommand{\PZB}{\HepAntiParticle{\PZ}{}{}\Xspace}
\DeclareRobustCommand{\myPAB}{\HepAntiParticle{\PA}{}{}\Xspace}
\DeclareRobustCommand{\OM}{\HepAntiParticle{\PM}{}{}\Xspace}
\DeclareRobustCommand{\OMf}{\HepAntiParticle{\PM}{}{\Pf}\Xspace}
\DeclareRobustCommand{\OMs}{\HepAntiParticle{\PM}{}{\,2}\Xspace}
\DeclareRobustCommand{\OMq}{\HepAntiParticle{\PM}{}{\,4}\Xspace}
\DeclareRobustCommand{\OMzs}{\HepAntiParticle{\PM}{\,0}{\,2}\Xspace}
\DeclareRobustCommand{\OMzq}{\HepAntiParticle{\PM}{\,0}{\,4}\Xspace}
\DeclareRobustCommand{\OMH}{\HepAntiParticle{\PM}{\,\PH}{}\Xspace}
\DeclareRobustCommand{\OMHs}{\HepAntiParticle{\PM}{\,\PH}{\,2}\Xspace}
\DeclareRobustCommand{\OMHq}{\HepAntiParticle{\PM}{\,\PH}{\,4}\Xspace}
\DeclareRobustCommand{\phib}{\HepAntiParticle{\upphi}{}{}\Xspace}
\newcommand{\ACf}{\frac{\OMs}{\HSs}}
%
%
\newcommand{\myYM}{\rm{\scriptscriptstyle{YM}}}
\newcommand{\gfix}{{\mbox{\scriptsize gf}}}
\newcommand{\myFP}{\rm{\scriptscriptstyle{FP}}}
%
\newcommand{\fact}{{\mbox{\scriptsize fc}}}
\newcommand{\nfact}{{\mbox{\scriptsize nfc}}}
\newcommand{\spin}{{\mbox{\scriptsize spin}}}
\newcommand{\app}{{\mbox{\scriptsize app}}}
\newcommand{\fer}{{\mbox{\scriptsize fer}}}
%\newcommand{\mdiv}{{\mbox{\scriptsize div}}}
%
\DeclareRobustCommand{\OMzs}{\HepAntiParticle{\PM}{\,0}{\,2}\Xspace}
\DeclareRobustCommand{\PM}{\HepParticle{M}{}{}\Xspace}
%
\newcommand{\rmD}{\mathrm{D}}
\newcommand{\bh}{\beta_{\mathrm{h}}}
\newcommand{\bhb}{\overline{\beta}_{\mathrm{h}}}
\newcommand{\RL}{\mathrm{R}_{\Lambda}}
%\newcommand{\Ddmu}{\ssD^{(\leftrightarrow)}_{\mu}}
\newcommand{\Ddmu}{\mrD^{(\leftrightarrow)}_{\mu}}
\newcommand{\ddmu}{{\stackrel{\leftrightarrow}{\partial}}_{\mu}}
\newcommand{\drmu}{{\stackrel{\rightarrow}{\partial}}_{\mu}}
\newcommand{\dlmu}{{\stackrel{\leftarrow}{\partial}}_{\mu}}
%
\newcommand{\Mbs}{M^2}
\newcommand{\Mbc}{M^3}
\newcommand{\Mbq}{M^4}
\newcommand{\mzb}{M_0}
\newcommand{\Mzbs}{M^2_0}
\newcommand{\Mzbq}{M^q_0}
%
\newcommand{\apLWt}{a^{(3)}_{\upphi\,\sPL\,\scriptscriptstyle{\PW}}}
%
\newcommand{\apLldQ}{a_{\upphi\,\PL\Pl\PQd\PQQ}}
\newcommand{\apN}{a_{\upphi\,\PN}}
\newcommand{\aplVA}{a_{\upphi\,\Pl\,\scriptscriptstyle{\PV\PA}}}
\newcommand{\apLVA}{a_{\upphi\,\sPL\,\scriptscriptstyle{\PV\PA}}}
\newcommand{\apLA}{\mra_{\upphi\,\sPL\,\scriptscriptstyle{\PA}}}
\newcommand{\apLV}{\mra_{\upphi\,\sPL\,\scriptscriptstyle{\PV}}}
\newcommand{\apuVA}{a_{\upphi\,\PQu\,\scriptscriptstyle{\PV\PA}}}
\newcommand{\apdVA}{a_{\upphi\,\PQd\,\scriptscriptstyle{\PV\PA}}}
\newcommand{\apUVA}{a_{\upphi\,\sPQU\,\scriptscriptstyle{\PV\PA}}}
\newcommand{\apDVA}{a_{\upphi\,\sPQD\,\scriptscriptstyle{\PV\PA}}}
%
\newcommand{\apWAB}{a_{\upphi\,\scriptscriptstyle{\PW\PA\PB}}}
\newcommand{\apWAD}{a_{\upphi\,\scriptscriptstyle{\PW\PA\PD}}}
%
\newcommand{\alpBox}{a_{\Pl\,\upphi\,\scriptscriptstyle{\Box}}}
\newcommand{\aLpBox}{a_{\sPL\,\upphi\,\scriptscriptstyle{\Box}}}
\newcommand{\aupBox}{a_{\PQu\,\upphi\,\scriptscriptstyle{\Box}}}
\newcommand{\adpBox}{a_{\PQd\,\upphi\,\scriptscriptstyle{\Box}}}
%
\newcommand{\aQW}{a_{\scriptscriptstyle{\PQQ\PW}}}
\newcommand{\aAA}{a_{\scriptscriptstyle{\PAA}}}
\newcommand{\aZZ}{a_{\scriptscriptstyle{\PZZ}}}
\newcommand{\aAZ}{a_{\scriptscriptstyle{\PAZ}}}
\newcommand{\ap}{a_{\upphi}}
\newcommand{\apBox}{a_{\upphi\,\scriptscriptstyle{\Box}}}
\newcommand{\apWB}{\mra_{\upphi\,\scriptscriptstyle{\PW\PB}}}
\newcommand{\apWBa}{a^{(a)}_{\upphi\,\scriptscriptstyle{\PW\PB}}}
\newcommand{\apWDpB}{a^{(+)}_{\upphi\,\scriptscriptstyle{\PW\PD\PB}}}
\newcommand{\apWDmB}{a^{(-)}_{\upphi\,\scriptscriptstyle{\PW\PD\PB}}}
\newcommand{\apBW}{a_{\upphi\,\scriptscriptstyle{\PB\PW}}}
\newcommand{\apWA}{a_{\upphi\,\scriptscriptstyle{\PW\PA}}}
\newcommand{\apWZ}{a_{\upphi\,\scriptscriptstyle{\PW\PZ}}}
\newcommand{\apB}{\mra_{\upphi\,\scriptscriptstyle{\PB}}}
\newcommand{\apW}{\mra_{\upphi\,\scriptscriptstyle{\PW}}}
\newcommand{\apD}{a_{\upphi\,\scriptscriptstyle{\PD}}}
\newcommand{\aptD}{a^{(2)}_{\upphi\,\scriptscriptstyle{\PD}}}
\newcommand{\apDB}{a_{\upphi\,\scriptscriptstyle{\PD\PB}}}
\newcommand{\apG}{a_{\upphi\,\scriptscriptstyle{\PG}}}
%
\newcommand{\aqp}{a_{\PQq\,\upphi}}
\newcommand{\alp}{a_{\Pl\,\upphi}}
\newcommand{\aup}{a_{\PQu\,\upphi}}
\newcommand{\atp}{a_{\PQt\,\upphi}}
\newcommand{\adp}{a_{\PQd\,\upphi}}
\newcommand{\abp}{a_{\PQb\,\upphi}}
%--
\newcommand{\atG}{a_{\PQt\,\Pg}}
\newcommand{\abG}{a_{\PQb\,\Pg}}
%--
\newcommand{\aNa}{a^{(1)}_{\ssN}}
\newcommand{\aNb}{a^{(2)}_{\ssN}}
\newcommand{\aNc}{a^{(3)}_{\ssN}}
%
\newcommand{\aLp}{a_{\sPL\,\upphi}}
\newcommand{\aUp}{a_{\sPQU\,\upphi}}
\newcommand{\aDp}{a_{\sPQD\,\upphi}}
%
\newcommand{\apWDm}{a^{(-)}_{\upphi\,\scriptscriptstyle{\PW\PD}}}
\newcommand{\apWDp}{a^{(+)}_{\upphi\,\scriptscriptstyle{\PW\PD}}}
%
\newcommand{\auG}{a_{\PQu\,\scriptscriptstyle{\PG}}}
\newcommand{\adG}{a_{\PQd\,\scriptscriptstyle{\PG}}}
%
\newcommand{\atW}{a_{\PQt\,\scriptscriptstyle{\PW}}}
\newcommand{\auW}{a_{\PQu\,\scriptscriptstyle{\PW}}}
\newcommand{\atB}{a_{\PQt\,\scriptscriptstyle{\PB}}}
\newcommand{\auB}{a_{\PQu\,\scriptscriptstyle{\PB}}}
\newcommand{\afWB}{a_{\Pf\,\scriptscriptstyle{\PW\PB}}}
\newcommand{\auWB}{a_{\PQu\,\scriptscriptstyle{\PW\PB}}}
\newcommand{\auBW}{a_{\PQu\,\scriptscriptstyle{\PB\PW}}}
\newcommand{\atWB}{a_{\PQt\,\scriptscriptstyle{\PW\PB}}}
\newcommand{\atBW}{a_{\PQt\,\scriptscriptstyle{\PB\PW}}}
%
\newcommand{\aUW}{a_{\sPQU\,\scriptscriptstyle{\PW}}}
\newcommand{\aUB}{a_{\sPQU\,\scriptscriptstyle{\PB}}}
\newcommand{\aUWB}{a_{\sPQU\,\scriptscriptstyle{\PW\PB}}}
\newcommand{\aUBW}{a_{\sPQU\,\scriptscriptstyle{\PB\PW}}}
%
\newcommand{\abW}{a_{\PQb\,\scriptscriptstyle{\PW}}}
\newcommand{\adW}{a_{\PQd\,\scriptscriptstyle{\PW}}}
\newcommand{\abB}{a_{\PQb\,\scriptscriptstyle{\PB}}}
\newcommand{\adB}{a_{\PQd\,\scriptscriptstyle{\PB}}}
\newcommand{\adWB}{a_{\PQd\,\scriptscriptstyle{\PW\PB}}}
\newcommand{\adBW}{a_{\PQd\,\scriptscriptstyle{\PB\PW}}}
\newcommand{\abWB}{a_{\PQb\,\scriptscriptstyle{\PW\PB}}}
\newcommand{\abBW}{a_{\PQb\,\scriptscriptstyle{\PB\PW}}}
%
\newcommand{\aDW}{a_{\sPQD\,\scriptscriptstyle{\PW}}}
\newcommand{\aDB}{a_{\sPQD\,\scriptscriptstyle{\PB}}}
\newcommand{\aDWB}{a_{\sPQD\,\scriptscriptstyle{\PW\PB}}}
\newcommand{\aDBW}{a_{\sPQD\,\scriptscriptstyle{\PB\PW}}}
%
\newcommand{\afW}{a_{\Pf\,\scriptscriptstyle{\PW}}}
\newcommand{\afB}{a_{\Pf\,\scriptscriptstyle{\PB}}}
%
\newcommand{\alW}{\mra_{\Pl\,\scriptscriptstyle{\PW}}}
\newcommand{\alB}{\mra_{\Pl\,\scriptscriptstyle{\PB}}}
\newcommand{\alWB}{\mra_{\Pl\,\scriptscriptstyle{\PW\PB}}}
\newcommand{\alBW}{a_{\Pl\,\scriptscriptstyle{\PB\PW}}}
%
%\newcommand{\aLW}{a_{\sPL\,\scriptscriptstyle{\PW}}}
%\newcommand{\aLB}{a_{\sPL\,\scriptscriptstyle{\PB}}}
%\newcommand{\aLWB}{\mra_{\sPL\,\scriptscriptstyle{\PW\PB}}}
%\newcommand{\aLBW}{a_{\sPL\,\scriptscriptstyle{\PB\PW}}}
%
\newcommand{\aplWt}{a^{(3)}_{\upphi\,\Pl\,\scriptscriptstyle{\PW}}}
\newcommand{\apqWt}{a^{(3)}_{\upphi\,\PQq\,\scriptscriptstyle{\PW}}}
\newcommand{\apQWt}{a^{(3)}_{\upphi\,\sPQQ\,\scriptscriptstyle{\PW}}}
%
\newcommand{\aplV}{\mra_{\upphi\,\Pl\,\scriptscriptstyle{\PV}}}
\newcommand{\aplA}{\mra_{\upphi\,\Pl\,\scriptscriptstyle{\PA}}}
\newcommand{\apfV}{a_{\upphi\,\Pf\,\scriptscriptstyle{\PV}}}
\newcommand{\apuV}{a_{\upphi\,\PQu\,\scriptscriptstyle{\PV}}}
\newcommand{\aptV}{a_{\upphi\,\PQt\,\scriptscriptstyle{\PV}}}
\newcommand{\apfA}{a_{\upphi\,\Pf\,\scriptscriptstyle{\PA}}}
\newcommand{\apuA}{a_{\upphi\,\PQu\,\scriptscriptstyle{\PA}}}
\newcommand{\aptA}{a_{\upphi\,\PQt\,\scriptscriptstyle{\PA}}}
\newcommand{\apUV}{a_{\upphi\,\sPQU\,\scriptscriptstyle{\PV}}}
\newcommand{\apUA}{a_{\upphi\,\sPQU\,\scriptscriptstyle{\PA}}}
\newcommand{\apdV}{a_{\upphi\,\PQd\,\scriptscriptstyle{\PV}}}
\newcommand{\apbV}{a_{\upphi\,\PQb\,\scriptscriptstyle{\PV}}}
\newcommand{\apdA}{a_{\upphi\,\PQd\,\scriptscriptstyle{\PA}}}
\newcommand{\apbA}{a_{\upphi\,\PQb\,\scriptscriptstyle{\PA}}}
\newcommand{\apDV}{a_{\upphi\,\sPQD\,\scriptscriptstyle{\PV}}}
\newcommand{\apDA}{a_{\upphi\,\sPQD\,\scriptscriptstyle{\PA}}}
\newcommand{\apn}{a_{\upphi\,\PGn}}
%
\newcommand{\aplo}{a^{(1)}_{\upphi\,\Pl}}
\newcommand{\aplt}{a^{(3)}_{\upphi\,\Pl}}
\newcommand{\apqo}{a^{(1)}_{\upphi\,\PQq}}
\newcommand{\apQo}{a^{(1)}_{\upphi\,\sPQQ}}
\newcommand{\apqt}{a^{(3)}_{\upphi\,\PQq}}
%
\newcommand{\apLo}{a^{(1)}_{\upphi\,\sPL}}
\newcommand{\apLt}{a^{(3)}_{\upphi\,\sPL}}
\newcommand{\apQt}{a^{(3)}_{\upphi\,\sPQQ}}
%
\newcommand{\apq}{a_{\upphi\,\PQq}}
\newcommand{\apu}{a_{\upphi\,\PQu}}
\newcommand{\apd}{a_{\upphi\,\PQd}}
\newcommand{\apl}{\mra_{\upphi\,\Pl}}
%
\newcommand{\apQ}{a_{\upphi\,\sPQQ}}
\newcommand{\apU}{a_{\upphi\,\sPQU}}
\newcommand{\apDq}{a_{\upphi\,\sPQD}}
\newcommand{\apL}{a_{\upphi\,\sPL}}
%
\newcommand{\aLldQ}{a_{\sPL\,\Pl\,\PQd\,\sPQQ}}
\newcommand{\aoQuQd}{a^{(1)}_{\sPQQ\,\PQu\,\sPQQ\,\PQd}}
\newcommand{\aoLlQu}{a^{(1)}_{\sPL\,\Pl\,\sPQQ\,\PQu}}
%
\newcommand{\bfun}[3]{\mrB_0^{\fin}\lpar #1\,;\,#2\,,\,#3\rpar}
\newcommand{\sbfun}[2]{\mrB_0^{\fin}\lpar #1\,,\,#2\rpar}
\newcommand{\bfunp}[3]{\mrB_{0\mathrm{p}}^{\fin}\lpar #1\,;\,#2\,,\,#3\rpar}
\newcommand{\bfuns}[3]{\mrB_{0\mathrm{s}}^{\fin}\lpar #1\,;\,#2\,,\,#3\rpar}
%
\newcommand{\zbfunp}[2]{\mrB_{0\mathrm{p}}^{\fin}\lpar \,#1\,,\,#2\rpar}
\newcommand{\zbfuns}[2]{\mrB_{0\mathrm{s}}^{\fin}\lpar \,#1\,,\,#2\rpar}
%
\newcommand{\ssp}{\mathrm{p}}
%
\newcommand{\WC}[1]{\ssW_{#1}}
\newcommand{\WCr}[1]{\ssW^{\ren}_{#1}}
%
\newcommand{\vtqs}{\mathrm{v}^2_{\PQt}}
\newcommand{\vbqs}{\mathrm{v}^2_{\PQb}}
\newcommand{\vtq}{\mathrm{v}_{\PQt}}
\newcommand{\vbq}{\mathrm{v}_{\PQb}}
%
\newcommand{\vqu}{\mathrm{v}_{\PQu}}
\newcommand{\vqd}{\mathrm{v}_{\PQd}}
\newcommand{\vle}{\mathrm{v}_{\Pl}}
\newcommand{\vqus}{\mathrm{v}^2_{\PQu}}
\newcommand{\vqds}{\mathrm{v}^2_{\PQd}}
\newcommand{\vles}{\mathrm{v}^2_{\Pl}}
%
\newcommand{\vple}{\mathrm{v}^{+}_{\Pl}}
\newcommand{\vpqu}{\mathrm{v}^{+}_{\PQu}}
\newcommand{\vpqd}{\mathrm{v}^{+}_{\PQd}}
\newcommand{\vmle}{\mathrm{v}^{-}_{\Pl}}
\newcommand{\vmqu}{\mathrm{v}^{-}_{\PQu}}
\newcommand{\vmqd}{\mathrm{v}^{-}_{\PQd}}
%
%\newcommand{\sla}[1]{/\!\!\!#1}
\newcommand{\sla}[1]{/\!\!\!\!\!#1}
%
\newcommand{\OPI}{1\mathrm{PI}}
\newcommand{\OPR}{1\mathrm{PR}}
%
\newcommand{\IR}{1\mathrm{IR}}
%
\newcommand{\DUV}{\Delta_{\mathrm{UV}}}
\newcommand{\DIR}{\Delta_{\mathrm{IR}}}
\newcommand{\LUV}{{\mathrm L}_{\mathrm{UV}}}
\newcommand{\DUVM}{\Delta_{\mathrm{UV}}\lpar \mws \rpar}
%
\newcommand{\cfun}[6]{\ssC_0\lpar #1\,,\,#2\,,\,#3\,;\,#4\,,\,#5\,,\,#6\rpar}
\newcommand{\cfunf}[6]{\ssC^{\fin}_0\lpar #1\,,\,#2\,,\,#3\,;\,#4\,,\,#5\,,\,#6\rpar}
\newcommand{\scfun}[2]{\ssC_0\lpar #1\,;\,#2\rpar}
%
%\newcommand{\sbfun}[2]{b^{\fin}_0\lpar #1\,,\,#2 \rpar}
\newcommand{\afun}[1]{a^{\fin}_0\lpar #1 \rpar}
%
\newcommand{\hyp}[4]{{}_2\,\mrF_1\lpar #1\,,\,#2\,;\,#3\,;\,#4\rpar}
%
\newcommand{\xptvi}{x^6_{\PQt}}
\newcommand{\xpbvi}{x^6_{\PQb}}
%
\newcommand{\xphvi}{x^6_{\sPH}}
\newcommand{\xphq}{x^4_{\sPH}}
\newcommand{\xpuq}{x^4_{\PQu}}
\newcommand{\xptq}{x^4_{\PQt}}
\newcommand{\xpdq}{x^4_{\PQd}}
\newcommand{\xpbq}{x^4_{\PQb}}
\newcommand{\xplq}{x^4_{\Pl}}
%
\newcommand{\xpss}{x^2_{\sPS}}
\newcommand{\xphs}{x^2_{\sPH}}
\newcommand{\xpus}{x^2_{\PQu}}
\newcommand{\xpts}{x^2_{\PQt}}
\newcommand{\xpds}{x^2_{\PQd}}
\newcommand{\xpbs}{x^2_{\PQb}}
\newcommand{\xpls}{x^2_{\Pl}}
\newcommand{\xpuc}{x^3_{\PQu}}
\newcommand{\xpdc}{x^3_{\PQd}}
\newcommand{\xplc}{x^3_{\Pl}}
%
\newcommand{\xpUs}{x^2_{\sPQU}}
\newcommand{\xpDs}{x^2_{\sPQD}}
\newcommand{\xpLs}{x^2_{\sPL}}
%--
\newcommand{\xps}{x_{\sPS}}
\newcommand{\xph}{x_{\sPH}}
\newcommand{\xpu}{x_{\PQu}}
\newcommand{\xpd}{x_{\PQd}}
\newcommand{\xpl}{x_{\Pl}}
%
\DeclareRobustCommand{\xog}{x^{(1)}_{\gen}}
\DeclareRobustCommand{\xtg}{x^{(2)}_{\gen}}
\DeclareRobustCommand{\vog}{v^{(1)}_{\gen}}
\DeclareRobustCommand{\vtg}{v^{(2)}_{\gen}}
%--
%
\newcommand{\sumg}{\sum_{\ggen}}
%
\newcommand{\xpUq}{x^4_{\sPQU}}
\newcommand{\xpDq}{x^4_{\sPQD}}
\newcommand{\xpLq}{x^4_{\sPL}}
\newcommand{\xpLc}{x^3_{\sPL}}
\newcommand{\xpUc}{x^3_{\sPQU}}
\newcommand{\xpDc}{x^3_{\sPQD}}
%
\newcommand{\xpU}{x_{\sPQU}}
\newcommand{\xpD}{x_{\sPQD}}
\newcommand{\xpL}{x_{\sPL}}
%
\newcommand{\vpus}{\mathrm{v}^2_{\PQu}}
\newcommand{\vpds}{\mathrm{v}^2_{\PQd}}
\newcommand{\vpls}{\mathrm{v}^2_{\Pl}}
%
\newcommand{\vpu}{\mathrm{v}_{\PQu}}
\newcommand{\vpd}{\mathrm{v}_{\PQd}}
\newcommand{\vpl}{\mathrm{v}_{\Pl}}
%
\newcommand{\mcA}{\mathcal{A}}
\newcommand{\mcB}{\mathcal{B}}
\newcommand{\mcC}{\mathcal{C}}
\newcommand{\mcD}{\mathcal{D}}
\newcommand{\mcE}{\mathcal{E}}
%--
\newcommand{\mcO}{\mathcal{O}}
\newcommand{\mcP}{\mathcal{P}}
\newcommand{\mcM}{\mathcal{M}}
\newcommand{\mcS}{\mathcal{S}}
\newcommand{\mcH}{\mathcal{H}}
\newcommand{\mcV}{\mathcal{V}}
\newcommand{\mcF}{\mathcal{F}}
\newcommand{\mcG}{\mathcal{G}}
\newcommand{\mcW}{\mathcal{W}}
\newcommand{\mcT}{\mathcal{T}}
\newcommand{\mcU}{\mathcal{U}}
\newcommand{\mcX}{\mathcal{X}}
\newcommand{\mcY}{\mathcal{Y}}
\newcommand{\mcR}{\mathcal{R}}
\newcommand{\mcL}{\mathcal{L}}
\newcommand{\mcZ}{\mathcal{Z}}
%
\newcommand{\myNG}{{\mathrm N}_{\gen}}
\newcommand{\LR}{{\mathrm L}_{\ssR}}
\newcommand{\Lir}{{\mathrm L}_{\mathrm{ir}}}
\newcommand{\mrdim}{\mathrm{dim}}
\newcommand{\cdim}{\mathrm{codim}}
%
\newcommand{\UVsl}{{\mathrm C}^{\sPL}_{\mathrm{UV}}}
\newcommand{\UVst}{{\mathrm C}^{\sPQU}_{\mathrm{UV}}}
\newcommand{\UVsb}{{\mathrm C}^{\sPQD}_{\mathrm{UV}}}
%
\newcommand{\lzs}{\lambda^2_{\sPZ}}
\newcommand{\lz}{\lambda_{\sPZ}}
\newcommand{\lws}{\lambda^2_{\sPW}}
\newcommand{\lw}{\lambda_{\sPW}}
%
\newcommand{\lazs}{\lambda^2_{\sPA\sPZ}}
\newcommand{\lzzs}{\lambda^2_{\sPZ\sPZ}}
\newcommand{\lwws}{\lambda^2_{\sPW\sPW}}
%
\newcommand{\laz}{\lambda_{\sPA\sPZ}}
\newcommand{\lzz}{\lambda_{\sPZ\sPZ}}
\newcommand{\lww}{\lambda_{\sPW\sPW}}
%
\newcommand{\WFHs}{\mrW^{(6)}_{\PH}}
\newcommand{\WFWs}{\mrW^{(6)}_{\PW}}
\newcommand{\degfs}{\mathrm{d}\mcZ^{(6)}_g}
\newcommand{\dMfs}{\mathrm{d}\mcZ^{(6)}_{\mw}}
%
\newcommand{\WFH}{\mrW^{(4)}_{\PH}}
\newcommand{\WFA}{\mrW^{(4)}_{\PA}}
\newcommand{\WFZ}{\mrW^{(4)}_{\PZ}}
\newcommand{\WFW}{\mrW^{(4)}_{\PW}}
\newcommand{\degf}{\mathrm{d}\mcZ^{(4)}_g}
\newcommand{\dMf}{\mathrm{d}\mcZ^{(4)}_{\mw}}
\newcommand{\dcthf}{\mathrm{d}\mcZ^{(4)}_c}
%
\newcommand{\WFZt}{\mrW^{(4)}_{\PZ\,\mid\,\PQt}}
\newcommand{\WFZb}{\mrW^{(4)}_{\PZ\,\mid\,\PQb}}
\newcommand{\WFZW}{\mrW^{(4)}_{\PZ\,\mid\,\PW}}
\newcommand{\WFZrf}{{\overline{\sum}}_{\gen}\,\mrW^{(4)}_{\PZ\,\mid\,\Pf}}
%
\newcommand{\WFHt}{\mrW^{(4)}_{\PH\,\mid\,\PQt}}
\newcommand{\WFHb}{\mrW^{(4)}_{\PH\,\mid\,\PQb}}
\newcommand{\WFHW}{\mrW^{(4)}_{\PH\,\mid\,\PW}}
\newcommand{\WFHtb}{\mrW^{(4)}_{\PH\,\mid\,\PQt,\PQb}}
%
\newcommand{\dMff}{\sum_{\gen}\,\mathrm{d}\mcZ^{(4)}_{M\,\mid\,\Pf}}
\newcommand{\dMfW}{\mathrm{d}\mcZ^{(4)}_{M\,\mid\,\PW}}
\newcommand{\dMftb}{\mathrm{d}\mcZ^{(4)}_{M\,\mid\,\PQt,\PQb}}
\newcommand{\dMfrf}{{\overline{\sum}}_{\gen}\,\mathrm{d}\mcZ^{(4)}_{M\,\mid\,\Pf}}
%
\newcommand{\degfrf}{\sum_{\gen}\,\mathrm{d}\mcZ^{(4)}_{g\,\mid\,\Pf}}
\newcommand{\degfW}{\mathrm{d}\mcZ^{(4)}_{g\,\mid\,\PW}}
\newcommand{\degftb}{\mathrm{d}\mcZ^{(4)}_{g\,\mid\,\PQt,\PQb}}
\newcommand{\degff}{\sum_{\gen}\,\mathrm{d}\mcZ^{(4)}_{g\,\mid\,\Pf}}
%
\newcommand{\dcthft}{\mathrm{d}\mcZ^{(4)}_{\ctw\,\mid\,\PQt}}
\newcommand{\dcthfb}{\mathrm{d}\mcZ^{(4)}_{\ctw\,\mid\,\PQb}}
\newcommand{\dcthfrf}{{\overline{\sum}}_{\gen}\,\mathrm{d}\mcZ^{(4)}_{\ctw\,\mid\,\Pf}}
\newcommand{\dcthfW}{\mathrm{d}\mcZ^{(4)}_{\ctw\,\mid\,\PW}}
%
\newcommand{\WFWtb}{\mrW^{(4)}_{\PW\,\mid\,\PQt,\PQb}}
\newcommand{\WFWW}{\mrW^{(4)}_{\PW\,\mid\,\PW}}
\newcommand{\WFWrf}{{\overline{\sum}}_{\gen}\,\mrW^{(4)}_{\PW\,\mid\,\Pf}}
%
\newcommand{\Dg}{\Delta g}
%
\newcommand{\spc}{\,,}
\newcommand{\spp}{\,\,.}
%
\newcommand{\gds}{g_{_6}}
%
\newcommand{\blueref}[1]{{\color{NavyBlue}{#1}}}
\newcommand{\redeq}[1]{{\color{BrickRed}{#1}}}
%
\newcommand{\proA}[1]{\Delta_{\sPA}(#1)}
\newcommand{\proZ}[1]{\Delta_{\sPZ}(#1)}
%
\newcommand{\DR}{\mathrm{DR}}
\newcommand{\SR}{\mathrm{SR}}
\newcommand{\NR}{\mathrm{NR}}
%
\newcommand{\sPAZ}{{\scriptscriptstyle{\PA\PZ}}}
\newcommand{\bmidl}{\Bigr|\Xspace}
\newcommand{\bmidr}{\Xspace\Bigr|}
\newcommand{\proZb}[1]{{\overline{\Delta}}_{\sPZ}(#1)}
\newcommand{\muV}{\mathswitch{\mu_{\sPV}}}
\newcommand{\muVs}{\mathswitch{\mu^2_{\sPV}}}
\newcommand{\gamV}{\mathswitch{\gamma_{\sPV}}}
\newcommand{\gamVs}{\mathswitch{\gamma^2_{\sPV}}}
\newcommand{\reg}{{\mbox{\scriptsize reg}}}
\newcommand{\xord}{{\mbox{\scriptsize{ord}}}}
\newcommand{\phys}{{\mbox{\scriptsize{phys}}}}
%
\newcommand{\muZ}{\mathswitch{\mu_{\sPZ}}}
\newcommand{\muZs}{\mathswitch{\mu^2_{\sPZ}}}
\newcommand{\gamZ}{\mathswitch{\gamma_{\sPZ}}}
\newcommand{\gamZs}{\mathswitch{\gamma^2_{\sPZ}}}
%
\newcommand{\PO}{\mathrm{\scriptscriptstyle{PO}}}
%
\newcommand{\egam}[1]{\Gamma(#1)}
%
\DeclareRobustCommand{\PWpL}{\HepParticle{\PW}{\PL}{+}\Xspace}
\DeclareRobustCommand{\PWmL}{\HepParticle{\PW}{\PL}{-}\Xspace}
%
\DeclareRobustCommand{\PAe}{\HepAntiParticle{\Pe}{}{}\Xspace}
%--
\newcommand{\tcif}{\mathswitch {I^{(3)}_{\Pf}}}
%
\newcommand{\sft}{{\mbox{\scriptsize soft}}}
%
\newcommand{\gsix}{\mathswitch {g_{_6}}}
%
\newcommand{\gve}{{{g^{\Pe}_{\sPV}}}}
\newcommand{\gae}{{{g^{\Pe}_{\sPA}}}}
\newcommand{\gvf}{{{g^{\Pf}_{\sPV}}}}
\newcommand{\gaf}{{{g^{\Pf}_{\sPA}}}}
\newcommand{\Qe}{Q_{\Pe}}
\newcommand{\Qf}{Q_{\Pf}}
\newcommand{\Qes}{Q^2_{\Pe}}
\newcommand{\Qfs}{Q^2_{\Pf}}
%
\newcommand{\sone}{s_{_1}}
\newcommand{\stwo}{s_{_2}}
\newcommand{\sPAA}{{\scriptscriptstyle{\PA\PA}}}
\newcommand{\spinub}[1]{\mybar{{\mathrm{u}}}_{#1}}
\newcommand{\spinu}[1]{{\mathrm{u}}_{#1}}
\newcommand{\spinv}[1]{{\mathrm{v}}_{#1}}
\newcommand{\mcQ}{\mathcal{Q}}
\newcommand{\sPHZ}{{\scriptscriptstyle{\PH\PZ}}}
%
\newcommand{\spinubL}[1]{\mybar{{\mathrm{u}}}_{#1\,\scriptscriptstyle{\mrL}}}
\newcommand{\spinubR}[1]{\mybar{{\mathrm{u}}}_{#1\,\scriptscriptstyle{\mrR}}}
\newcommand{\spinvL}[1]{{\mathrm{v}}_{#1\,\scriptscriptstyle{\mrL}}}
\newcommand{\spinvR}[1]{{\mathrm{v}}_{#1\,\scriptscriptstyle{\mrR}}}
%
\newcommand{\sbe}{\sin\beta}
\newcommand{\cbe}{\cos\beta}
\newcommand{\sbes}{\sin^2\beta}
\newcommand{\cbes}{\cos^2\beta}
\newcommand{\sbeq}{\sin^4\beta}
\newcommand{\cbeq}{\cos^4\beta}
\newcommand{\tbe}{\tan\beta}
\newcommand{\tbes}{\tan^2\beta}
\newcommand{\stbe}{\sin(2\,\beta)}
\newcommand{\ctbe}{\cos(2\,\beta)}
\newcommand{\sab}{\sin(\alpha - \beta)}
\newcommand{\cab}{\cos(\alpha - \beta)}
\newcommand{\sabs}{\sin^2(\alpha - \beta)}
\newcommand{\cabs}{\cos^2(\alpha - \beta)}
%
\newcommand{\Msb}{{\overline M}}
\newcommand{\Msbs}{{\overline M}^2}
\newcommand{\lb}{{\overline \lambda}}
\newcommand{\tb}{{\overline t}}
\newcommand{\mrFb}{{\overline \mrF}}
%
\newcommand{\dbe}{\delta_{\beta}}
\newcommand{\dal}{\delta_{\alpha}}
%
\DeclareRobustCommand{\PHpm}{\HepParticle{\PH}{}{\,\pm}\Xspace}
\DeclareRobustCommand{\PAz}{\HepParticle{\PA}{}{\,0}\Xspace}
\DeclareRobustCommand{\PHp}{\HepParticle{\PH}{}{+}\Xspace}
\DeclareRobustCommand{\PHm}{\HepParticle{\PH}{}{-}\Xspace}
%
\DeclareRobustCommand{\PKz}{\HepParticle{\upPhi}{0}{2}\Xspace}
\DeclareRobustCommand{\PKh}{\HepParticle{\upPhi}{\Ph}{2}\Xspace}
%
\DeclareRobustCommand{\PKzs}{\HepParticle{\upPhi}{0}{4}\Xspace}
\DeclareRobustCommand{\PKhs}{\HepParticle{\upPhi}{\Ph}{4}\Xspace}
%
\DeclareRobustCommand{\PKzc}{\HepParticle{\upPhi}{0}{6}\Xspace}
\DeclareRobustCommand{\PKhc}{\HepParticle{\upPhi}{\Ph}{6}\Xspace}
%
\DeclareRobustCommand{\CDmu}{\HepParticle{\PD}{\mu}{}\Xspace}
\DeclareRobustCommand{\pumu}{\HepParticle{\partial}{}{\mu}\Xspace}
\DeclareRobustCommand{\punu}{\HepParticle{\partial}{}{\nu}\Xspace}
\DeclareRobustCommand{\pdmu}{\HepParticle{\partial}{\mu}{}\Xspace}
\DeclareRobustCommand{\pdnu}{\HepParticle{\partial}{\nu}{}\Xspace}
\DeclareRobustCommand{\pdal}{\HepParticle{\partial}{\alpha}{}\Xspace}
%
%\DeclareRobustCommand{\PuPz}{\HepParticle{\upPhi}{0}{}\Xspace}
%\DeclareRobustCommand{\PuPh}{\HepParticle{\upPhi}{\Ph}{}\Xspace}
%\DeclareRobustCommand{\PuPzd}{\HepParticle{\upPhi}{0}{\dagger}\Xspace}
%\DeclareRobustCommand{\PuPhd}{\HepParticle{\upPhi}{\Ph}{\dagger}\Xspace}
%%
%\DeclareRobustCommand{\PKz}{\PuPzd\,\PuPz}
%\DeclareRobustCommand{\PKh}{\PuPhd\,\upPhi_{\Ph}}
%\DeclareRobustCommand{\PKzs}{\lpar \PuPzd\,\PuPz \rpar^2}
%\DeclareRobustCommand{\PKhs}{\lpar \PuPhd\,\PuPh \rpar^2}
%\DeclareRobustCommand{\PKzc}{\lpar \PuPzd\,\PuPz \rpar^3}
%\DeclareRobustCommand{\PKhc}{\lpar \PuPhd\,\PuPh \rpar^3}
%--
\newcommand{\pdmuPh}{\pdmu\,\Ph}
\newcommand{\pdmuPpz}{\pdmu\,\Ppz}
\newcommand{\pdmuPpp}{\pdmu\,\Ppp}
\newcommand{\pdmuPpm}{\pdmu\,\Ppm}
\newcommand{\pdmuPKh}{\pdmu\,\PKh}
\newcommand{\pdmuPKhs}{\pdmu\,\PKh\,\pdmu\,\PKh}
\newcommand{\PkinA}{\pdmu\,\PAdnu\,\pdmu\,\PAdnu}
\newcommand{\PkinZ}{\pdmu\,\PZdnu\,\pdmu\,\PZdnu}
\newcommand{\PkinW}{\pdmu\,\PWpdnu\,\pdmu\,\PWmdnu}
\newcommand{\PDQu}{\CDmu\,\PQu}
\newcommand{\PDQd}{\CDmu\,\PQd}
\newcommand{\PdivA}{\pdmu\,\PAdmu}
\newcommand{\PdivZ}{\pdmu\,\PZdmu}
\newcommand{\PdivWp}{\pdmu\,\PWpdmu}
\newcommand{\PdivWm}{\pdmu\,\PWmdmu}
\newcommand{\PWpnumu}{\pdnu\,\PWpdmu}
\newcommand{\PWmnumu}{\pdnu\,\PWmdmu}
\newcommand{\PdAnumu}{\pdnu\,\PAdmu}
\newcommand{\PdZnumu}{\pdnu\,\PZdmu}
\newcommand{\PdXmmu}{\pdmu\,\PXm}
\newcommand{\PdXpmu}{\pdmu\,\PXp}
\newcommand{\PdYamu}{\pdmu\,\PYa}
\newcommand{\PdYzmu}{\pdmu\,\PYz}
\newcommand{\PZdmus}{\PZdmu\,\PZdmu}
\newcommand{\PdmuPpp}{\CDmu\,\Ppp}
\newcommand{\PdmuPpm}{\CDmu\,\Ppm}
\newcommand{\PdmuPppm}{\CDmu\,\Ppp\,\CDmu\,\Ppm}
\newcommand{\PdAXmmu}{\pdmu\,\PAXm}
\newcommand{\PdAXpmu}{\pdmu\,\PAXp}
\newcommand{\PdAYamu}{\pdmu\,\PAYa}
\newcommand{\PdAYzmu}{\pdmu\,\PAYz}
\newcommand{\PdWpnumu}{\pdnu\,\PWpmu}
\newcommand{\PdWmnumu}{\pdnu\,\PWmmu}
%
\newcommand{\MSB}{{\overline{\mathrm{MS}}}}
%
\newcommand{\Nf}{\mathbb{N}}
\newcommand{\Rf}{\mathbb{R}}
\newcommand{\Cf}{\mathbb{C}}
\newcommand{\Zf}{\mathbb{Z}}
\newcommand{\dsimp}[1]{\int\,dS_{#1}}
\newcommand{\dsimpg}[1]{\int\,dS^{\gamma}_{#1}}
\newcommand{\dcub}[1]{\int\,dC_{#1}}
\newcommand{\dsimpd}{\int\,dS^d_2}
\newcommand{\dcubs}[2]{\int\,dCS\lpar #1\,;\,#2 \rpar}
\newcommand{\pd}{\scriptscriptstyle{+}}
\newcommand{\ppd}{\scriptscriptstyle{++}}
\newcommand{\pppd}{\scriptscriptstyle{+++}}
\newcommand{\mrLi}{{\mathrm{Li}}}
\newcommand{\tHs}{\mu_{\mathrm{DR}}}
%
\newcommand{\gammab}{{\bar{\gamma}}}
\newcommand{\gammah}{{\hat{\gamma}}}
\newcommand{\barnm}{\overline{\nu}_{\mu}}
\newcommand{\supMSB}[1]{{#1}^{\mbox{$\overline{\scriptscriptstyle MS}$}}}
\newcommand{\refig}[1]{\autoref{#1}}

\newcommand{\tDdr}{1/{\bar{\varepsilon}}}
\newcommand{\hsp}{\hspace{.5mm}}%
  \def\captionof{\caption@teststar\caption@of{\caption*}\caption}

\newcommand{\Ecut}{\mrE_{\mrc}}
\newcommand{\tcut}{t_{\mrc}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

